Groups of PL-homeomorphisms admitting non-trivial invariant characters

We show that several classes of groups G of PL-homeomorphisms of the real line admit non-trivial homomorphisms from G to the additive group of reals that are fixed by every automorphism of G. The classes of groups enjoying the stated property include the generalisations of Thompson's group F studied by K. S. Brown, M. Stein, S. Cleary, and Bieri-Strebel but also the class of groups investigated by Bieri-Neumann-Strebel in [BNS87, Theorem 8.1]. It follows that every automorphism of a group in one of these classes has infinitely many associated twisted conjugacy classes.

==> Definitions.tex <==
%
\makeatletter
%
%
\DeclareMathOperator{\ab}{ab}
\DeclareMathOperator{\add}{add}
\DeclareMathOperator{\Aff}{Aff}
\DeclareMathOperator{\Ann}{Ann}
\DeclareMathOperator{\Aut}{Aut}
%   B
\DeclareMathOperator{\BPL}{BPL}
\DeclareMathOperator{\BS}{BS}

%   C
\DeclareMathOperator{\can}{can}
\DeclareMathOperator{\card}{card}
\DeclareMathOperator{\codim}{codim}
\DeclareMathOperator{\coker}{coker}
\DeclareMathOperator{\colim}{colim}
\DeclareMathOperator{\core}{core}
%   D
\DeclareMathOperator{\Der}{Der}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\defi}{def}
\DeclareMathOperator{\dom}{dom}
\DeclareMathOperator{\Dr}{Dr}
%   E
\DeclareMathOperator{\edg}{E}
\DeclareMathOperator{\e}{e}
\DeclareMathOperator{\End}{End}
\DeclareMathOperator{\Ext}{Ext}
%   F
\DeclareMathOperator{\face}{face}
\DeclareMathOperator{\FF}{FF}
\DeclareMathOperator{\fg}{fg}
\DeclareMathOperator{\Fit}{Fit}
\DeclareMathOperator{\Fix}{Fix}
\DeclareMathOperator{\FP}{FP}
\DeclareMathOperator{\Frat}{Frat}
%   G

\DeclareMathOperator{\gp}{gp}
\DeclareMathOperator{\GL}{GL}
%   H
\DeclareMathOperator{\Cohom}{H}
\DeclareMathOperator{\Hom}{Hom}
\DeclareMathOperator{\Homeo}{Homeo}
%  I
\newcommand{\id}{\mathbbm{1}}
\DeclareMathOperator{\im}{im}
\DeclareMathOperator{\Inn}{Inn}
\DeclareMathOperator{\Int}{int}
\DeclareMathOperator{\inv}{inv}
%   M
\DeclareMathOperator{\md}{md}
%  N
\newcommand{\norm}[1]{\| #1\|}
%  O
\DeclareMathOperator{\odd}{odd}
%  P
\DeclareMathOperator{\PL}{PL}
%  Q
\DeclareMathOperator{\Quot}{Quot}
%   R
\DeclareMathOperator{\res}{res}
\DeclareMathOperator{\rk}{rk}

%    S
\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\SL}{SL}
\DeclareMathOperator{\sing}{sing}
\DeclareMathOperator{\myspan}{span}
\DeclareMathOperator{\stab}{St}
\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\SUPP}{SUPP}
\DeclareMathOperator{\sym}{sym}
\DeclareMathOperator{\Sym}{Sym}
\DeclareMathOperator{\sgp}{sgp}
\DeclareMathOperator{\smd}{smd}
%  T
\DeclareMathOperator{\Tor}{Tor}
\DeclareMathOperator{\tor}{tor}
\DeclareMathOperator{\TPL}{TPL}
%   V
\DeclareMathOperator{\Val}{Val}
\DeclareMathOperator{\ver}{V}
%
%%
%%
\def\B{\mathbb{B}} 
\def\C{\mathbb{C}}
\def\E{\mathbb{E}}
\def\F{\mathbb{F}}
\def\G{\mathbb{G}}
\def\H{\mathbb{H}}
\def\I{\mathbb{I}}
\def\K{\mathbb{K}}
\def\L{\mathbb{L}}
\def\M{\mathbb{M}}
\def\N{\mathbb{N}}
\def\P{\mathbb{P}}
\def\Q{\mathbb{Q}}
\def\R{\mathbb{R}}
\def\s{\mathbb{S}}
\def\U{\mathbb{U}}
\def\Z{\mathbb{Z}}
%
%
%% Calligraphic letters
\let\@@angstroem=\AA    
\let\angstroem=\@@angstroem
\def\AA{\mathcal{A}}
\def\BB{\mathcal{B}}
\def\CC{\mathcal{C}}
\def\DD{\mathcal{D}}
\def\EE{\mathcal{E}}
\def\FF{\mathcal{F}}
\def\GG{\mathcal{G}}
\def\HH{\mathcal{H}}
\def\II{\mathcal{I}}
\def\JJ{\mathcal{J}}
\def\KK{\mathcal{K}}
\def\LL{\mathcal{L}}
\def\MM{\mathcal{M}}
\def\NN{\mathcal{N}}
\def\OO{\mathcal{O}}
\def\PP{\mathcal{P}}
\def\QQ{\mathcal{Q}}
\def\RR{\mathcal{R}}
\def\SS{\mathcal{S}}
\def\TT{\mathcal{T}}
\def\UU{\mathcal{U}}
\def\VV{\mathcal{V}}
\def\WW{\mathcal{W}}
\def\XX{\mathcal{X}}
\def\YY{\mathcal{Y}}
\def\ZZ{\mathcal{Z}}
%%
%
%% Morphisms
%
\newcommand{\mono}{\rightarrowtail}
\newcommand{\incl}{\hookrightarrow}
\newcommand{\epi}{\twoheadrightarrow}
\newcommand{\iso}{\stackrel{\sim}{\longrightarrow}}
\newcommand{\isoinv}{\stackrel{\sim}{\longleftarrow}}
%
% Useful abbreviations (see LaTeX Companion, page 80)
%
\newcommand{\cf}{cf. \xspace}
\newcommand{\eg}{e.g., \xspace}
\newcommand{\ie}{i.e., \xspace}
\newcommand{\etc}{etc. \@\xspace}
\newcommand{\Ka}{K{\"a}hler}
% command for left conjugation
\newcommand{\act}[3]{{}^{#1} \mspace{#2mu} #3}
\newcommand{\actN}[1]{{}^{#1}}
%
%
%
\makeatother
\endinput
